DifferSketching: How Differently Do People Sketch 3D Objects?

Multiple sketch datasets have been proposed to understand how people draw 3D objects. However, such datasets are often of small scale and cover a small set of objects or categories. In addition, these datasets contain freehand sketches mostly from expert users, making it difficult to compare the drawings by expert and novice users, while such comparisons are critical in informing more effective sketch-based interfaces for either user groups. These observations motivate us to analyze how differently people with and without adequate drawing skills sketch 3D objects. We invited 70 novice users and 38 expert users to sketch 136 3D objects, which were presented as 362 images rendered from multiple views. This leads to a new dataset of 3,620 freehand multi-view sketches, which are registered with their corresponding 3D objects under certain views. Our dataset is an order of magnitude larger than the existing datasets. We analyze the collected data at three levels, i.e., sketch-level, stroke-level, and pixel-level, under both spatial and temporal characteristics, and within and across groups of creators. We found that the drawings by professionals and novices show significant differences at stroke-level, both intrinsically and extrinsically. We demonstrate the usefulness of our dataset in two applications: (i) freehand-style sketch synthesis, and (ii) posing it as a potential benchmark for sketch-based 3D reconstruction. Our dataset and code are available at https://chufengxiao.github.io/DifferSketching/.

==> Figures/fig_basic_hist.tex <==
\begin{figure}[t]{
    \centering
    \subfloat[Difference in stroke number]{
        \includegraphics[width=.49\linewidth]{Figures/revised_SA/strokeNum.pdf}
    }
    \subfloat[Difference in drawing length]{
        \includegraphics[width=.49\linewidth]{Figures/revised_SA/drawPath.pdf}
    }
    \caption{Two histograms of the differences between the drawings by professional and novice users across all the categories on stroke number and drawing length (accumulated stroke length). % respectively. 
    The differences are computed by subtracting the total value of five novice users from that of five professional users for the same prompt (P-N).}
    \label{fig:basic_hist}
    }
\end{figure}

==> Figures/fig_reg_qual.tex <==
\begin{figure}[htb]{
    \centering
    \includegraphics[width=\linewidth]{Figures/stroke_stat/reg_qual.pdf}
    \caption{}
    \label{fig:reg_qual}
    }
\end{figure}

==> Figures/fig_stroke_alignRate.tex <==
\begin{figure}[htb]{
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/stroke_stat/StrokePrecision.pdf}
    \caption{Stroke precision of the stroke-level registered results for each category.}
    \label{fig:stroke_precision}
    }
\end{figure}

==> Figures/tab_three_levels.tex <==
\begin{table}
    \footnotesize
    \caption{The statistics for three levels of registration {differences to the corresponding tracings in terms of Rotation ($R$), Translation ($T$) and Scale ($S$)}. We show $mean/standard ~deviation$ pairs on the two groups for each metric in three analysis levels. Note that we only evaluated the valid drawings / strokes that are registered correctly. The valid counts are also presented here.
    We have `-' for the pixel-level rotation and scale, since these values cannot be evaluated at the pixel level. 
    }
    \begin{tabular}[width=0.9\textwidth]{c|c|c|c|c|c}
         \hline
         Level & Skill & Count & $R$ ( $\degree$ ) & $T$ (pixel) & $S$ \\
         \hline
         \multirow{2}{*}{Sketch-level} & N  & 1680 & 5.06 / 5.52 & 121.03 / 89.76 & 0.89 / 0.20 \\
         & P & 1778 & 3.57 / 4.58 & 86.68 / 70.11 & 0.95 / 0.14  \\
         \hline
         \multirow{2}{*}{Stroke-level} & N  & $\sim$59.9K & 12.83 / 14.54 & 222.58 / 198.23 & 1.02 / 0.39 \\
         & P & $\sim$89.4K & 10.60 / 11.98 & 184.53 / 172.22 &  1.01 / 0.32 \\
         \hline
         \multirow{2}{*}{Pixel-level} & N & $\sim$11.2M  & - & 8.67 / 14.14 & -  \\
         & P & $\sim$12.6M & - & 5.17 / 8.94 & - \\
         \hline
    \end{tabular}
     
    \label{tab:three_levels}
\end{table}
